Directional and Quasi-Omnidirectional Indoor Channel Measurements at Upper 6 GHz

This paper presents wideband indoor channel measurements and measurement-based statistical modeling of channel parameters in the upper 6 GHz (U6G) band using directional and quasi-omnidirectional antenna pairs. Measurements span 6.425-7.125 GHz at 32 matched positions per configuration in an open hall and an L-shaped corridor. System calibration and frequency-dependent peak-gain normalization retain antenna radiation-pattern weighting. Close-in and floating-intercept models are fitted to line-of-sight (LOS) and non-LOS (NLOS) path loss, respectively. Shadow-fading residuals, RMS delay spread (DS), and equivalent K factors derived from power delay profiles are characterized. LOS exponents range from 1.98 to 2.14. Despite similar attenuation slopes, directional links exhibit smaller LOS residuals and DS and higher equivalent K factors. Hall DS medians are 1.78 and 36.52 ns for directional and quasi-omnidirectional links. Corridor NLOS slopes are -1.12 and 2.54, respectively, while DS ordering varies by position. These results characterize antenna-dependent parameters for U6G indoor channels.

==> fig1_measurement_system.tex <==
\begin{tikzpicture}[
  scale=\FigureCoordinateScale,
  font=\FigureTextFont,
  block/.style={draw, rounded corners=1.5pt, text width=1.80cm,
                minimum height=0.76cm, align=center, fill=blue!5},
  rf/.style={block, fill=orange!10},
  ant/.style={block, fill=green!10},
  link/.style={-Latex, semithick},
  link label/.style={font=\FigureTextFont, align=center, fill=white,
                     inner sep=1pt},
  every node/.style={inner sep=2.5pt}
]
\node[block] (vnatx) at (0,1.25) {R\&S ZNA67\\VNA Tx port};
\node[rf] (eo) at (3.15,1.25) {electrical-to-\\optical};
\node[block] (fiber) at (6.30,1.25) {optical\\fiber link};
\node[rf] (oe) at (6.30,0) {optical-to-\\electrical/RF};
\node[ant] (tx) at (3.15,0) {Tx\\antenna};
\node[ant] (rx) at (0,0) {Rx\\antenna};
\node[block] (vnarx) at (0,-1.25) {R\&S ZNA67\\VNA Rx port};

\draw[link] (vnatx) -- node[link label, above=5pt]{frequency\\sweep} (eo);
\draw[link] (eo) -- (fiber);
\draw[link] (fiber) -- (oe);
\draw[link] (oe) -- (tx);
\draw[link] (tx) -- node[link label, above=1pt]{indoor\\channel} (rx);
\draw[link] (rx) -- (vnarx);
\draw[dashed, gray] (-1.10,2.15) rectangle (7.40,-1.78);

\end{tikzpicture}


==> measurement_photo_panel.tex <==
% Vector overlays preserve the original photograph and its existing crop.
\begin{tikzpicture}[
  scale=\FigureCoordinateScale,
  photoLabel/.style={font=\FigureTextFont,
    fill=white,fill opacity=.92,text opacity=1,inner sep=1.5pt,
    rounded corners=.7pt},
  photoArrow/.style={-Latex,white,line width=.55pt}]
\path[use as bounding box] (0,0) rectangle (5,2.65);
\node[inner sep=0pt,transform shape] at (2.5,1.325)
  {\includegraphics[width=5cm,height=2.65cm,trim={0 105bp 0 105bp},clip]{measurement_photo.jpg}};
\node[photoLabel,anchor=north west] (pcLabel) at (.10,2.55) {Control PC};
\draw[photoArrow] (pcLabel.south east)--(1.27,1.89);
\node[photoLabel,anchor=south west] (vnaLabel) at (.10,.15) {VNA sounder};
\draw[photoArrow] (vnaLabel.north east)--(1.53,1.11);
\node[photoLabel,anchor=north east] (antLabel) at (4.90,2.55)
  {Directional antennas};
\draw[photoArrow] (antLabel.south west)--(3.17,2.25);
\draw[photoArrow] (antLabel.south)--(3.98,2.22);
\end{tikzpicture}

